Addressing Label Leakage in Knowledge Tracing Models

Knowledge Tracing (KT) is concerned with predicting students' future performance on learning items in intelligent tutoring systems. Learning items are tagged with skill labels called knowledge concepts (KCs). Many KT models expand the sequence of item-student interactions into KC-student interactions by replacing learning items with their constituting KCs. This approach addresses the issue of sparse item-student interactions and minimises the number of model parameters. However, we identified a label leakage problem with this approach. The model's ability to learn correlations between KCs belonging to the same item can result in the leakage of ground truth labels, which leads to decreased performance, particularly on datasets with a high number of KCs per item. In this paper, we present methods to prevent label leakage in knowledge tracing (KT) models. Our model variants that utilize these methods consistently outperform their original counterparts. This further underscores the impact of label leakage on model performance. Additionally, these methods enhance the overall performance of KT models, with one model variant surpassing all tested baselines on different benchmarks. Notably, our methods are versatile and can be applied to a wide range of KT models.

==> sections/LSTM.tex <==
\section*{Long Short-Term Memory (LSTM)}
%TODO fix this section
To make this work self-contained, we describe the LSTM architecture. LSTMs were introduced to mitigate the vanishing or exploding gradient problems that occur when training RNNs where the gradient becomes extremely small or explode to large values especially when applied to long sequences.

An LSTM network is composed of a series of cells, each of which contains three main components:
\begin{itemize}
    \item \textbf{Input gate} ($i_t$): Controls the extent to which new information flows into the cell.
    \item \textbf{Forget gate} ($f_t$): Decides what portion of the cell state should be forgotten.
    \item \textbf{Output gate} ($o_t$): Determines how much of the cell state should be output to the next time step.
\end{itemize}

The core of an LSTM cell is its cell state ($C_t$), which is modified by the input, forget, and output gates. The following equations describe the operations within an LSTM cell at time step $t$:

\begin{align*}
    f_t &= \sigma(W_f \cdot [h_{t-1}, x_t] + b_f) \\
    i_t &= \sigma(W_i \cdot [h_{t-1}, x_t] + b_i) \\
    o_t &= \sigma(W_o \cdot [h_{t-1}, x_t] + b_o) \\
    \tilde{C}_t &= \tanh(W_C \cdot [h_{t-1}, x_t] + b_C) \\
    C_t &= f_t \cdot C_{t-1} + i_t \cdot \tilde{C}_t \\
    h_t &= o_t \cdot \tanh(C_t)
\end{align*}

where $\sigma$ is the sigmoid activation function, $\tanh$ is the hyperbolic tangent activation function, $x_t$ is the input at time step $t$, $h_{t-1}$ is the hidden state from the previous time step, and $W$ and $b$ are the weight matrices and bias vectors, respectively.

LSTMs mitigate the vanishing gradient problem commonly encountered in standard RNNs, enabling them to capture long-term dependencies in the data.


==> sections/arxiv_intro.tex <==
Knowledge Tracing (KT) models are a fundamental component for personalisation and recommendation in intelligent tutoring systems (ITS). Some models can also provide diagnostic outputs regarding the skills or concepts covered in the coursework, such as a student's mastery of these concepts. These concepts are typically listed by the ITS and referred to as Knowledge Concepts (KCs).

Due to the large number of questions available in ITS and the limited student-question interactions, many KT models use KCs to address sparsity issues \cite{pykt,akt}. The use of KCs also helps to reduce parameter size. To achieve this, each question can be unfolded into its constituent KCs, creating a new KC-student interaction sequence instead of question-student interactions. This approach is similar to that used in Deep Knowledge Tracing (DKT) \cite{dkt} and Attentive Knowledge Tracing (AKT) \cite{akt}.

When expanding the KC-student sequence, KC items of the same question precede one another. This can lead to data leakage during evaluation and cause misleading results \cite{pykt}. To ensure proper evaluation of models, each group of KCs that constitute a question should be evaluated independently of each other \cite{pykt}. However, this approach can be computationally expensive for some models.


Additionally, we noticed that models trained using this method can also learn to leak data between KCs of the same question and thus suffer from degrading performance. This problem is more pronounced when dealing with datasets that have a high average number of KCs per question. It is worth noting that classical models that do not learn dependency between different KCs, such as \textit{Bayesian Knowledge Tracing} (BKT), do not suffer from this problem. Therefore, this paper focuses solely on deep knowledge tracing models (DLKT) that can learn complex dependencies between KCs.



Furthermore, the length of the KC-student interaction sequence is longer than the question-student sequence, which is often ignored in benchmark comparisons that do not enforce a fixed sequence length of questions across different KT models. Most benchmarks use datasets with a small average number of KCs per question. As a result, the difference in length between the expanded KC sequence and the original question sequence is usually minimal. However, in this paper, we use datasets with a higher average number of KCs per question to address the mentioned problems.


The contributions of this work are:
\begin{itemize}
    \item We provide empirical evidence for data leakage during training of such models.
    \item In addition, we introduce a number of methods to prevent data leakage. 
    \item Lastly, we perform all benchmarks under the same sequence lengths across different models. 
    \item We publish our implementations as an open source framework.
\end{itemize}

%Despite the reported success of these models, the literature was inconsistent about evaluating these models against eachother\docite{}. Some of these evaluation problems were adressed in \docite{}. One problem that has not been adressed is evaluating different models on the same benchmarks but with different sequence window size...
. %One problem is that the same benchmark has not been adressed is that different models have been tested on  

%Beside data leakage during evaluation, we have noticed that a lot of these models suffer from data leakage during training... we provide a general framework to remidy this issue with minmum adjustment to these models.
%Despite the reported success of these models, there is divergence between benchmark resulsts in the literature

%Knowledge tracing models have been plagued with evaluation divergence between published research... Some of these problems have been adressed in \docite{}.





==> sections/attention.tex <==
\subsubsection*{Monotonic Attention Mechanism}
%TODO fix the intro


AKT monotonic attention is based on the scaled dot-product attention which is a fundamental part in models such as the Transformers\cite{transformer}. The original scaled dot-product attention operates by computing attention scores, which determine the importance of each input item relative to the other items. This mechanism is particularly effective in capturing dependencies in sequences.
 
A scaled dot-product attention takes a sequence of queries, keys, and values. Each key corresponds to a single value. Queries and keys are vectors of dimension $d_k$ while values are captured by vectors of dimension $d_v$. For each query index $i$, a score, $s_{i,j}$, is computed for each value index $j$ as follows:
\[
s_{i,j} = \frac{\mathbf{q}_i^T \cdot \mathbf{k}_j}{\sqrt{d_k}}
\]
Where $q_i$ and $k_j$ are query and key vectors correspondingly. Where $d_k$ is used as a scaling factor to prevent the dot products from becoming excessively large. To obtain the attention weight \( w_{i,j} \) for the query \( \mathbf{q}_i \) with respect to the key \( \mathbf{k}_j \), the softmax function is applied to the attention scores:
\[
w_{i,j} = \text{Softmax}(s_{i,j}) = \frac{\exp\left(s_{i,j}\right)}{\sum_j \exp\left(s_{i,j}\right)}
\]
These weights $w_{i,j}$ are then used to compute the weighted sum of the value vectors $v_j$, which forms the output of the attention mechanism:

$$
\text{Attention}(\mathbf{q}_i, K, V) = \sum_{j} w_{i,j} \mathbf{v}_j
$$

This approach allows the model to dynamically focus on different parts of the input sequence, effectively capturing long-range dependencies.

The monotonic attention computes different scores $s_{i,j}'$  %that are used to compute the attention weights  

$$s_{i, j}'=\frac{\exp (-\theta \cdot d(t, \tau)) \cdot q_\tau^{\top} k_\tau}{\sqrt{d_k}}$$, 

	where $\theta > 0$ is a learnable decay rate parameter. $d(i, j)$ is a context-aware distance measure that is computed as follows:	
%\begin{equation}
%\begin{aligned} 
%d(t, \tau) & =|t-\tau| \cdot \sum_{t^{\prime}=\tau+1} \gamma_{t, t^{\prime}} \\
%
%	  \gamma_{t, t^{\prime}} & =\frac{\exp \left(\s_{i,j}\right)}{\sum_{1 \leq \tau^{\prime} \leq t} s_{i,j})}, \forall t^{\prime} \leq t .
%	\end{aligned}
%\end{equation}


%\begin{equation}
%\begin{aligned} 
%d(t, \tau) & = |t-\tau| \cdot \sum_{t^{\prime}=\tau+1}^t \gamma_{t, t^{\prime}} \\
%\gamma_{t, t^{\prime}} & = \frac{\exp \left(s_{i,j}\right)}{\sum_{1 \leq \tau^{\prime} \leq t} s_{i,j}}, \forall t^{\prime} \leq t .
%\end{aligned}
%\end{equation}


\begin{equation}
\begin{aligned} 
d(i, j) & = |i - j| \cdot \sum_{i^{\prime}=j+1}^i \gamma_{i, i^{\prime}} \\
\gamma_{i, i^{\prime}} & = \frac{\exp \left(s_{i,j}\right)}{\sum_{1 \leq j^{\prime} \leq i} s_{i,j}}, \forall i^{\prime} \leq i.
\end{aligned}
\end{equation}

	      where $s_{i,j}$ are the original scaled dot-product scores. The new monotonic attention weights are  $w_{i,j} = \text{Softmax}(s_{i,j}')$.
		  

		


